Distributed Resource Allocation with Multi-Agent Deep Reinforcement Learning for 5G-V2V Communication

We consider the distributed resource selection problem in Vehicle-to-vehicle (V2V) communication in the absence of a base station. Each vehicle autonomously selects transmission resources from a pool of shared resources to disseminate Cooperative Awareness Messages (CAMs). This is a consensus problem where each vehicle has to select a unique resource. The problem becomes more challenging when---due to mobility---the number of vehicles in vicinity of each other is changing dynamically. In a congested scenario, allocation of unique resources for each vehicle becomes infeasible and a congested resource allocation strategy has to be developed. The standardized approach in 5G, namely semi-persistent scheduling (SPS) suffers from effects caused by spatial distribution of the vehicles. In our approach, we turn this into an advantage. We propose a novel DIstributed Resource Allocation mechanism using multi-agent reinforcement Learning (DIRAL) which builds on a unique state representation. One challenging issue is to cope with the non-stationarity introduced by concurrently learning agents which causes convergence problems in multi-agent learning systems. We aimed to tackle non-stationarity with unique state representation. Specifically, we deploy view-based positional distribution as a state representation to tackle non-stationarity and perform complex joint behavior in a distributed fashion. Our results showed that DIRAL improves PRR by 20% compared to SPS in challenging congested scenarios.

==> discussions.tex <==
\section{Further Discussions}
\label{sec:discussions}

\subsection{Random velocity}
In all of the experiments, the positional distribution of the vehicles on the road is finite and expected. After the training, the model can generate one joint action for each positional distribution and each vehicle can apply its part of the action based on their view-based positional observation. We tested the model with the toy example also under random velocities.  At the end of the episode, each vehicle either accelerate(+0.1) or decelerate(-0.1) i.e. $\min(0.8 m/step, vel_t^i \pm \delta), \max(1.4 m/step, vel_t^i \pm \delta)$. Note that the periodicity of the CAM message is $100ms$ which leads to the variation of the velocity between $28.8kmph - 50.4kmph$ and every 2.5 seconds it either increase or decrease $3.6kmph$. The result in Figure \ref{fig:random_toy} shows that the algorithm can not reach the optimal policy but vehicles can still learn a sub-optimal policy(2 vehicles use separate resources, 2 same resources). However, the results can be improved further by integrating velocity as a part of the state feature $v_t^i \in s_t^i$. We leave this case as a part of the future work.
% NOTE: add figure

\subsection{Impact of LSTM layer}
We also analyzed the impact of the LSTM input layer on learning performance. Hence, the first LSTM layer is replaced by feedforward neural networks(FNN) as vanilla DQN. Scenario 6 i.e. 20 vehicles, 20 resources is exploited for comparing the performance of these two settings. The results in Figure \ref{fig:dqnvsdrqn} show that LSTM input layer enables learning whereas vanilla DQN with FNN as first later is now able to learn at all. LSTM layer captures the previous $m$ observations e.g. in our case $m=6$ instead of learning only from the last observation.
% NOTE: add figure
\subsection{Granularity of observations}
The performance of the proposed approach under different granularity i.e. $B$ differs is also examined. We observed that the optimal bin size $B$ is correlated with the number of vehicles in a scenario. Training performance of toy example and scenario 6 under various $B$ value is depicted in Figure \ref{fig:train_per_bin}. In general, the variance of the learning curve diminishes with increasing granularity.

\begin{figure*}
\begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=0.8\linewidth]{infocom2021_TVT/figures/results/paper_random_velocity_toy_example_b20.pdf} 
    \caption{Toy example under random velocity}
    \label{fig:random_toy}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  % include first image
  \includegraphics[width=0.8\linewidth]{infocom2021_TVT/figures/results/final_20ue_20r_500m_35kmph_dqn_vs_drqn.pdf}
    \caption{Scenario 6, Vanilla DQN vs DQN with LSTM}
    \label{fig:dqn_vs_drqn}
\end{subfigure}
\newline
\begin{subfigure}{.49\textwidth}
  \centering
  % include third image
  \includegraphics[width=0.8\linewidth]{infocom2021_TVT/figures/results/final_4ue_3r_toy_o_index_bin_sizes.pdf}  
  \caption{Scenario 1}
  \label{fig:sub-first}
\end{subfigure}
\begin{subfigure}{.49\textwidth}
  \centering
  % include fourth image
  \includegraphics[width=0.8\linewidth]{infocom2021_TVT/figures/results/final_20ue_20r_500m_35kmph_bin_size.pdf}  
  \caption{Scenario 6}
  \label{fig:sub-second}
\end{subfigure}
\caption{Training performance of different scenarios}
\label{fig:fig:train_per_further}
\end{figure*}


\subsection{Networked agents}
Our work can also be considered as a part of the networked agents in multi-agent deep reinforcement learning system in which agents exchange messages through a communication channel in order to maximize system objective. Communication in multi-agent reinforcement learning is a new emerging trend for cooperative and competitive settings \cite{DBLP:journals/corr/FoersterAFW16a, DBLP:journals/corr/abs-1802-08757, DBLP:journals/corr/abs-1902-01554}. In our system, each agent shares its neighboring positional table with the other agents to keep updated position information of each vehicle in the system. This positional information is later used to construct state of the agent. Note that, sharing positional information with other agents does not create extra burden on radio resources since we share the messages together with the CAM messages. Also, our work aligns with the latest 5G V2X standards, sharing information with other vehicles to assist their resource selection is also part of the 5G-V2X i.e.mode 2(b) standard \cite{R11809867}.



